Federated Learning with Partial Model Personalization

We consider two federated learning algorithms for training partially personalized models, where the shared and personal parameters are updated either simultaneously or alternately on the devices. Both algorithms have been proposed in the literature, but their convergence properties are not fully understood, especially for the alternating variant. We provide convergence analyses of both algorithms in the general nonconvex setting with partial participation and delineate the regime where one dominates the other. Our experiments on real-world image, text, and speech datasets demonstrate that (a) partial personalization can obtain most of the benefits of full model personalization with a small fraction of personal parameters, and, (b) the alternating update algorithm often outperforms the simultaneous update algorithm by a small but consistent margin.

==> figs/fedalt_dependent_rvs.tex <==
\begin{tikzpicture}
% \usetikzlibrary{arrows.meta}
% \usepackage[customcolors,shade]{hf-tikz}

\node[draw, color=black, fill=black!1, very thick, circle, minimum size=1.7cm] 
  (S) at (0, 2.5) {\fontfamily{cmss}\selectfont \Large $S^{(t)}$};

\node[draw, color=black, fill=red!10, very thick, circle, minimum size=1.5cm] (V) at (-2,0) 
{\fontfamily{cmss}\selectfont \Large $V^{(t+1)}$}; 
    
\node[draw, color=black, fill=blue!10, very thick, circle, minimum size=1.5cm] (u) at (2,0) 
{\fontfamily{cmss}\selectfont \Large $u^{(t+1)}$};  

\node[draw, color=black, very thick, fill=black!1,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1.5cm] (inp) at (0, -3) 
    {\fontfamily{cmss}\selectfont \Large 
    $\Big\langle
    \nabla_u F\big(u^{(t)}, \, 
    \tikzmarkin[set fill color=red!10,
set border color=black!0]{vv}(0.1,-0.25)(-0.1,0.6) V^{(t+1)}\tikzmarkend{vv}  \, \big),  \, \,
    \tikzmarkin[set fill color=blue!10,
set border color=black!0]{uu}(0.1,-0.25)(-0.1,0.6)u^{(t+1)}\tikzmarkend{uu} 
    \, - u^{(t)}
    \Big\rangle$
    };

\draw[-{Latex[width=4mm]}, very thick] (S) edge (V) ;
\draw[-{Latex[width=4mm]}, very thick] (S) edge (u) ;

\draw[-{Latex[width=4mm]}, very thick] (V) edge (inp) ;
\draw[-{Latex[width=4mm]}, very thick] (u) edge (inp) ;

\end{tikzpicture}


==> figs/fedalt_independent_rv.tex <==
\begin{tikzpicture}
% \usetikzlibrary{arrows.meta}
% \usepackage[customcolors,shade]{hf-tikz}

\node[draw, color=black, fill=black!1, very thick, circle, minimum size=1.7cm] 
  (S) at (0, 2.5) {\fontfamily{cmss}\selectfont \Large $S^{(t)}$};

\node[draw, color=black, fill=red!10, very thick, circle, minimum size=1.5cm] (V) at (-2,0) 
{\fontfamily{cmss}\selectfont \Large $V^{(t+1)}$}; 
    
\node[draw, color=black, fill=blue!10, very thick, circle, minimum size=1.5cm] (u) at (2,0) 
{\fontfamily{cmss}\selectfont \Large $u^{(t+1)}$};  

\node[draw, color=black, very thick, fill=black!1,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1.5cm] (inp) at (0, -3) 
    {\fontfamily{cmss}\selectfont \Large 
    $\Big\langle
    \nabla_u F\big(u^{(t)}, \, 
    \tikzmarkin[set fill color=yellow!45,
set border color=black!0]{vvv}(0.1,-0.25)(-0.1,0.6) \widetilde V^{(t+1)}\tikzmarkend{vvv}  \, \big),  \, \,
    \tikzmarkin[set fill color=blue!10,
set border color=black!0]{uuu}(0.1,-0.25)(-0.1,0.6)u^{(t+1)}\tikzmarkend{uuu} 
    \, - u^{(t)}
    \Big\rangle$
    };

\draw[-{Latex[width=4mm]}, very thick] (S) edge (V) ;
\draw[-{Latex[width=4mm]}, very thick] (S) edge (u) ;

% \draw[-{Latex[width=4mm]}, very thick] (V) edge (inp) ;
\draw[-{Latex[width=4mm]}, very thick] (u) edge (inp) ;

\end{tikzpicture}


==> figs/fedalt_main_1.tex <==
\begin{tikzpicture}
% \usetikzlibrary{arrows.meta}
% \usepackage[customcolors,shade]{hf-tikz}

\node[draw, color=black, fill=black!1, very thick, circle, minimum size=1.5cm] 
  (S) at (0, 1.5) {\fontfamily{cmss}\selectfont \Large $S^{(t)}$};

\node[draw, color=black, fill=red!10, very thick, circle, minimum size=1.5cm] (V) at (-3,0) 
{\fontfamily{cmss}\selectfont \Large $V^{(t+1)}$}; 
    
\node[draw, color=black, fill=blue!10, very thick, circle, minimum size=1.5cm] (u) at (3,0) 
{\fontfamily{cmss}\selectfont \Large $u^{(t+1)}$};  

\node[draw, color=black, very thick, fill=black!1,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1.5cm] (inp) at (0, -2) 
    {\fontfamily{cmss}\selectfont \Large 
    $\Big\langle
    \nabla_u F\big(u^{(t)}, \, 
    \tikzmarkin[set fill color=red!10,
set border color=black!0]{v1}(0.1,-0.25)(-0.1,0.6) V^{(t+1)}\tikzmarkend{v1}  \, \big),  \, \,
    \tikzmarkin[set fill color=blue!10,
set border color=black!0]{u1}(0.1,-0.25)(-0.1,0.6)u^{(t+1)}\tikzmarkend{u1} 
    \, - u^{(t)}
    \Big\rangle$
    };

\draw[-{Latex[width=4mm]}, very thick] (S) edge (V) ;
\draw[-{Latex[width=4mm]}, very thick] (S) edge (u) ;

\draw[-{Latex[width=4mm]}, very thick] (V) edge (inp) ;
\draw[-{Latex[width=4mm]}, very thick] (u) edge (inp) ;

\end{tikzpicture}


==> figs/fedalt_main_2.tex <==
\begin{tikzpicture}
% \usetikzlibrary{arrows.meta}
% \usepackage[customcolors,shade]{hf-tikz}

\node[draw, color=black, fill=black!1, very thick, circle, minimum size=1.5cm] 
  (S) at (0, 1.5) {\fontfamily{cmss}\selectfont \Large $S^{(t)}$};

\node[draw, color=black, fill=red!10, very thick, circle, minimum size=1.5cm] (V) at (-3,0) 
{\fontfamily{cmss}\selectfont \Large $V^{(t+1)}$}; 
    
\node[draw, color=black, fill=blue!10, very thick, circle, minimum size=1.5cm] (u) at (3,0) 
{\fontfamily{cmss}\selectfont \Large $u^{(t+1)}$};  

\node[draw, color=black, very thick, fill=black!1,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1.5cm] (inp) at (0, -2) 
    {\fontfamily{cmss}\selectfont \Large 
    $\Big\langle
    \nabla_u F\big(u^{(t)}, \, 
    \tikzmarkin[set fill color=yellow!45,
set border color=black!0]{v2}(0.1,-0.25)(-0.1,0.6) \widetilde V^{(t+1)}\tikzmarkend{v2}  \, \big),  \, \,
    \tikzmarkin[set fill color=blue!10,
set border color=black!0]{u2}(0.1,-0.25)(-0.1,0.6)u^{(t+1)}\tikzmarkend{u2} 
    \, - u^{(t)}
    \Big\rangle$
    };

\draw[-{Latex[width=4mm]}, very thick] (S) edge (V) ;
\draw[-{Latex[width=4mm]}, very thick] (S) edge (u) ;

% \draw[-{Latex[width=4mm]}, very thick] (V) edge (inp) ;
\draw[-{Latex[width=4mm]}, very thick] (u) edge (inp) ;

\end{tikzpicture}


==> figs/fedalt_main_3.tex <==
\begin{tikzpicture}
% \usetikzlibrary{arrows.meta}
% \usepackage[customcolors,shade]{hf-tikz}

\node[draw, color=black, fill=black!1, very thick, circle, minimum size=1.5cm] 
  (S) at (-2.5, 0) {\fontfamily{cmss}\selectfont \Large $S^{(t)}$};

\node[draw, color=black, fill=red!10, very thick, circle, minimum size=1.5cm] (V) at (0, 1.5) {\fontfamily{cmss}\selectfont \Large $V^{(t+1)}$}; 
    
\node[draw, color=black, fill=blue!10, very thick, circle, minimum size=1.5cm] (u) at (0, -1.5) 
{\fontfamily{cmss}\selectfont \Large $u^{(t+1)}$};  

\node[draw, color=black, very thick, fill=black!1,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1.5cm] (inp) at (7, 1) 
    {\fontfamily{cmss}\selectfont \Large 
    $\Big\langle
    \nabla_u F\big(u^{(t)}, \, 
    \tikzmarkin[set fill color=red!10,
set border color=black!0]{v1}(0.1,-0.25)(-0.1,0.6) V^{(t+1)}\tikzmarkend{v1}  \, \big),  \, \,
    \tikzmarkin[set fill color=blue!10,
set border color=black!0]{u1}(0.1,-0.25)(-0.1,0.6)u^{(t+1)}\tikzmarkend{u1} 
    \, - u^{(t)}
    \Big\rangle$
    };
    
\node[draw, color=black, very thick, fill=black!1,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1.5cm] (inp2) at (7, -1) 
    {\fontfamily{cmss}\selectfont \Large 
    $\Big\langle
    \nabla_u F\big(u^{(t)}, \, 
    \tikzmarkin[set fill color=yellow!45,
set border color=black!0]{v2}(0.1,-0.25)(-0.1,0.6) \widetilde V^{(t+1)}\tikzmarkend{v2}  \, \big),  \, \,
    \tikzmarkin[set fill color=blue!10,
set border color=black!0]{u2}(0.1,-0.25)(-0.1,0.6)u^{(t+1)}\tikzmarkend{u2} 
    \, - u^{(t)}
    \Big\rangle$
    };

\draw[-{Latex[width=4mm]}, very thick] (S) edge (V) ;
\draw[-{Latex[width=4mm]}, very thick] (S) edge (u) ;

\draw[-{Latex[width=4mm]}, very thick] (V) edge ([yshift=5pt]inp.west) ;
\draw[-{Latex[width=4mm]}, very thick] (u) edge ([yshift=-5pt]inp.west) ;
\draw[-{Latex[width=4mm]}, very thick] (u) edge (inp2.west) ;

\end{tikzpicture}


==> tables/aggregated/final_finetune_pretrained_stateful.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{2}{l}{StackOverflow (Transformer)} & \multicolumn{2}{l}{GLDv2 (ResNet)} & \multicolumn{2}{l}{EMNIST (ResNet)} \\
{} &                      PFL-AM &  PFL-SU &         PFL-AM &   PFL-SU &          PFL-AM &  PFL-SU \\
\midrule
Input Layer  &                     $-0.02$ &  $0.02$ &        $-0.00$ &   $0.00$ &          $0.05$ &  $0.03$ \\
Output Layer &                      $0.00$ &  $0.14$ &         $0.11$ &   $0.14$ &          $0.02$ &  $0.01$ \\
Adapter      &                      $0.00$ &  $0.22$ &        $-0.93$ &  $-0.20$ &          $0.14$ &  $0.12$ \\
\bottomrule
\end{tabular}


==> tables/aggregated/final_finetune_pretrained_stateless.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{2}{l}{StackOverflow (Transformer)} & \multicolumn{2}{l}{GLDv2 (ResNet)} & \multicolumn{2}{l}{EMNIST (ResNet)} \\
{} &                      PFL-AM &  PFL-SU &         PFL-AM &  PFL-SU &          PFL-AM &  PFL-SU \\
\midrule
Input Layer  &                      $0.74$ &  $0.70$ &         $0.15$ &  $0.12$ &          $0.02$ &  $0.01$ \\
Output Layer &                      $0.74$ &  $0.74$ &         $0.56$ &  $0.49$ &          $0.02$ &  $0.03$ \\
Adapter      &                      $0.67$ &  $0.65$ &         $6.60$ &  $5.19$ &          $0.17$ &  $0.14$ \\
\bottomrule
\end{tabular}


==> tables/expt_hyperparams.tex <==
\small
\begin{tabular}{cccccc}
\toprule
& Hyperparameter & StackOverflow & GLDv2 & EMNIST & LibriSpeech \\
\midrule

\multirow{9}{*}{Common} 
& Batch size & 64 & 64 & 32 & 32\\
& Devices per round & 50 & 50 & 10 & 50 \\
& Local epochs & 1 & 1 & 1 & 1\\
& Server Optimizer & FedAdam & FedAdam & FedAvg & FedAdam \\
& Client Optimizer & SGD & SGD & SGD & SGD  \\
& Global Scheduler & {Linear} & Linear & Exponential & Linear \\
& Warm up & $10\%$ of rounds & $10\%$ of rounds & N/A & $10\%$ of rounds\\
& LR decay rounds & N/A & N/A & $500$ & N/A\\
& Max. grad. norm. & $0.1$ & N/A & N/A & $0.25$ \\
\midrule
\multirow{3}{*}{\begin{tabular}{l} Non-personalized training \\ (step (a) of the pipeline)\end{tabular}} 
& \# Rounds & 1000 & 2500 & 2000 & 500  \\
& Server learning rate & $5\times 10^{-4}$ & $2 \times 10^{-4}$ & 1.0 & $10^{-3}$ \\
& Client learning rate & $1$ & $10^{-2}$ & $0.5$ & $10^{-2}$
\\
\midrule
\multirow{3}{*}{\begin{tabular}{l} Personalized training \\ (step (b) of the pipeline)\end{tabular}} 
& \# Rounds & 500 & 600 & 500 & 500 \\
& Server learning rate & $5\times 10^{-5}$ & $2 \times 10^{-5}$ & 1.0 & $10^{-3}$ \\
& Client learning rate & $10^{-1}$ & $10^{-3}$ & $10^{-2}$ & $10^{-2}$ \\
\midrule
\multirow{3}{*}{\begin{tabular}{l} Local finetuning \\ (step (c) of the pipeline)\end{tabular}} 
& \#Epochs & 5 & 5 & 5 & 5 \\
& Optimizer & SGD & SGD & SGD & SGD \\
& Client learning rate & $10^{-1}$ & $10^{-3}$ & $10^{-2}$ & $10^{-4}$ \\
\bottomrule
\end{tabular}

==> tables/final_finetune_pretrained_stateful.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{2}{c}{StackOverflow} & \multicolumn{2}{c}{GLDv2} & \multicolumn{2}{c}{EMNIST} \\
{} &          FedAlt &         FedSim &         FedAlt &         FedSim &         FedAlt &         FedSim \\
\midrule
Input Layer  &  $-0.06_{0.01}$ &  $0.04_{0.02}$ &  $0.12_{0.02}$ &  $0.17_{0.03}$ &  $0.12_{0.01}$ &  $0.12_{0.03}$ \\
Output Layer &   $0.00_{0.01}$ &  $0.25_{0.02}$ &  $0.49_{0.02}$ &  $0.57_{0.03}$ &  $0.09_{0.01}$ &  $0.09_{0.03}$ \\
Adapter      &   $0.01_{0.01}$ &  $0.40_{0.08}$ &  $0.14_{0.02}$ &  $0.17_{0.01}$ &  $0.27_{0.02}$ &  $0.33_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/final_finetune_pretrained_stateful2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{2}{c}{StackOverflow} & \multicolumn{2}{c}{GLDv2} & \multicolumn{2}{c}{EMNIST} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
{} &          FedAlt &         FedSim &         FedAlt &         FedSim &         FedAlt &         FedSim \\
\midrule
Input Layer  &  $-0.06_{0.01}$ &  $0.04_{0.02}$ &  $0.12_{0.02}$ &  $0.17_{0.03}$ &  $0.12_{0.01}$ &  $0.12_{0.03}$ \\
Output Layer &   $0.00_{0.01}$ &  $0.25_{0.02}$ &  $0.49_{0.02}$ &  $0.57_{0.03}$ &  $0.09_{0.01}$ &  $0.09_{0.03}$ \\
Adapter      &   $0.01_{0.01}$ &  $0.40_{0.08}$ &  $0.14_{0.02}$ &  $0.17_{0.01}$ &  $0.27_{0.02}$ &  $0.33_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/final_finetune_pretrained_stateless.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{2}{c}{StackOverflow} & \multicolumn{2}{c}{GLDv2} & \multicolumn{2}{c}{EMNIST} \\
{} &         FedAlt &         FedSim &          FedAlt &          FedSim &         FedAlt &         FedSim \\
\midrule
Input Layer  &  $0.86_{0.03}$ &  $1.00_{0.02}$ &   $0.44_{0.03}$ &   $0.42_{0.03}$ &  $0.11_{0.02}$ &  $0.10_{0.04}$ \\
Output Layer &  $1.08_{0.03}$ &  $1.10_{0.02}$ &   $1.47_{0.04}$ &   $1.46_{0.05}$ &  $0.15_{0.02}$ &  $0.11_{0.02}$ \\
Adapter      &  $0.84_{0.04}$ &  $0.88_{0.02}$ &  $11.68_{0.20}$ &  $10.42_{0.09}$ &  $0.46_{0.02}$ &  $0.42_{0.04}$ \\
\bottomrule
\end{tabular}


==> tables/final_finetune_pretrained_stateless2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{2}{c}{StackOverflow} & \multicolumn{2}{c}{GLDv2} & \multicolumn{2}{c}{EMNIST} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
{} &         FedAlt &         FedSim &          FedAlt &          FedSim &         FedAlt &         FedSim \\
\midrule
Input Layer  &  $0.86_{0.03}$ &  $1.00_{0.02}$ &   $0.44_{0.03}$ &   $0.42_{0.03}$ &  $0.11_{0.02}$ &  $0.10_{0.04}$ \\
Output Layer &  $1.08_{0.03}$ &  $1.10_{0.02}$ &   $1.47_{0.04}$ &   $1.46_{0.05}$ &  $0.15_{0.02}$ &  $0.11_{0.02}$ \\
Adapter      &  $0.84_{0.04}$ &  $0.88_{0.02}$ &  $11.68_{0.20}$ &  $10.42_{0.09}$ &  $0.46_{0.02}$ &  $0.42_{0.04}$ \\
\bottomrule
\end{tabular}


==> tables/main_nostd.tex <==
\begin{tabular}{l||l|lll|lll}
\toprule
{} & Non-personalized & \multicolumn{3}{c}{Full Model} & \multicolumn{3}{c}{$\partial$PFL} \\
{} &        Finetune &           Ditto &                   pFedMe &     Input Layer &    Output Layer &                  Adapter \\
\midrule
StackOverflow &   $23.82_{0.00}$ &  $25.20_{0.01}$ &  $25.20_{0.01}$ &  $\mathbf{25.21}_{0.01}$ &  $24.44_{0.01}$ &  $25.05_{0.01}$ &           $24.82_{0.01}$ \\
GLDv2         &   $51.43_{0.00}$ &  $62.85_{0.02}$ &  $62.85_{0.01}$ &           $62.92_{0.02}$ &  $53.94_{0.07}$ &  $56.64_{0.05}$ &  $\mathbf{66.41}_{0.06}$ \\
EMNIST        &   $93.18_{0.00}$ &  $94.13_{0.01}$ &  $94.13_{0.01}$ &  $\mathbf{94.13}_{0.01}$ &  $93.62_{0.04}$ &  $93.57_{0.05}$ &           $94.13_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/main_std.tex <==
\begin{tabular}{l||l|lll|lll}
\toprule
{} & Non-personalized & \multicolumn{3}{c}{Full Model} & \multicolumn{3}{c}{$\partial$PFL} \\
{} &        Finetune &           Ditto &                   pFedMe &     Input Layer &    Output Layer &                  Adapter \\
\midrule
StackOverflow &   $23.82_{0.00}$ &  $25.20_{0.01}$ &  $25.20_{0.01}$ &  $\mathbf{25.21}_{0.01}$ &  $24.44_{0.01}$ &  $25.05_{0.01}$ &           $24.82_{0.01}$ \\
GLDv2         &   $51.43_{0.00}$ &  $62.85_{0.02}$ &  $62.85_{0.01}$ &           $62.92_{0.02}$ &  $53.94_{0.07}$ &  $56.64_{0.05}$ &  $\mathbf{66.41}_{0.06}$ \\
EMNIST        &   $93.18_{0.00}$ &  $94.13_{0.01}$ &  $94.13_{0.01}$ &  $\mathbf{94.13}_{0.01}$ &  $93.62_{0.04}$ &  $93.57_{0.05}$ &           $94.13_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/main_std2.tex <==
%!TEX root = ../main.tex

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrrrr}
\toprule
{} & Non-pers. & \multicolumn{3}{c}{Full Model Personalization} & \multicolumn{3}{c}{Partial Model Personalization} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
    {} & FedAvg &        Finetune &           Ditto &                   pFedMe &     Input Layer &    Output Layer &                  Adapter \\
\midrule
StackOverflow &   $23.82$ &  \tabemph{} $\mathbf{25.20}_{0.01}$ &  \tabemph{} $\mathbf{25.20}_{0.01}$ &   \tabemph{} $\mathbf{25.21}_{0.01}$ &  $24.44_{0.01}$ &  $25.05_{0.01}$ &           $24.82_{0.01}$ \\
GLDv2         &   $51.43$ &  $62.85_{0.02}$ &  $62.85_{0.01}$ &           $62.92_{0.02}$ &  $53.94_{0.07}$ &  $56.64_{0.05}$ &   \tabemph{} $\mathbf{66.41}_{0.06}$ \\
EMNIST        &   $93.18$ &   \tabemph{} $\mathbf{94.13}_{0.01}$ &   \tabemph{} $\mathbf{94.13}_{0.01}$ &   \tabemph{} $\mathbf{94.13}_{0.01}$ &  $93.62_{0.04}$ &  $93.57_{0.05}$ &            \tabemph{} $\mathbf{94.13}_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/per_task/main_pretrained_stateful_emnist_resnetgn.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{l}{Mean Accuracy \%} & \multicolumn{3}{l}{10th Percentile Accuracy \%} \\
{} &         Finetune &            PFL-AM &   PFL-SU &                    Finetune &            PFL-AM &            PFL-SU \\
\midrule
Non-personalized &          $93.18$ &           $93.18$ &  $93.18$ &                     $86.11$ &           $86.11$ &           $86.11$ \\
Input Layer      &          $93.29$ &  $\mathbf{93.49}$ &  $93.37$ &            $\mathbf{86.21}$ &  $\mathbf{86.21}$ &  $\mathbf{86.21}$ \\
Output Layer     &          $93.37$ &  $\mathbf{93.43}$ &  $93.42$ &            $\mathbf{86.21}$ &  $\mathbf{86.21}$ &  $\mathbf{86.21}$ \\
Adapter          &          $93.65$ &  $\mathbf{93.92}$ &  $93.70$ &                     $86.84$ &  $\mathbf{87.80}$ &           $87.10$ \\
\bottomrule
\end{tabular}


==> tables/per_task/main_pretrained_stateful_gldv2_resnetgn.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{l}{Mean Accuracy \%} & \multicolumn{3}{l}{10th Percentile Accuracy \%} \\
{} &         Finetune &            PFL-AM &            PFL-SU &                    Finetune &            PFL-AM &            PFL-SU \\
\midrule
Non-personalized &          $67.19$ &           $67.19$ &           $67.19$ &                     $53.57$ &           $53.57$ &           $53.57$ \\
Input Layer      &          $67.62$ &  $\mathbf{73.40}$ &           $72.94$ &                     $53.90$ &  $\mathbf{59.46}$ &           $58.82$ \\
Output Layer     &          $69.02$ &  $\mathbf{75.62}$ &           $75.03$ &                     $55.74$ &  $\mathbf{62.16}$ &           $61.63$ \\
Adapter          &          $76.69$ &           $81.21$ &  $\mathbf{82.53}$ &                     $63.16$ &           $68.09$ &  $\mathbf{72.22}$ \\
\bottomrule
\end{tabular}


==> tables/per_task/main_pretrained_stateful_so_mini.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{l}{Mean Accuracy \%} & \multicolumn{3}{l}{10th Percentile Accuracy \%} \\
{} &          Finetune &            PFL-AM &   PFL-SU &                    Finetune &            PFL-AM &   PFL-SU \\
\midrule
Non-personalized   &           $23.82$ &           $23.82$ &  $23.82$ &                     $20.17$ &           $20.17$ &  $20.17$ \\
Input Layer        &  $\mathbf{24.95}$ &           $24.47$ &  $24.78$ &            $\mathbf{21.33}$ &           $20.71$ &  $21.14$ \\
Output Layer       &           $24.92$ &  $\mathbf{25.04}$ &  $24.77$ &            $\mathbf{21.41}$ &           $21.39$ &  $21.37$ \\
Adapter (dim=$16$) &           $24.71$ &  $\mathbf{24.81}$ &  $24.40$ &                     $21.21$ &  $\mathbf{21.24}$ &  $20.97$ \\
Adapter (dim=$64$) &           $24.73$ &  $\mathbf{24.85}$ &  $24.43$ &            $\mathbf{21.17}$ &           $21.15$ &  $21.04$ \\
\bottomrule
\end{tabular}


==> tables/per_task/main_pretrained_stateless_emnist_resnetgn.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{l}{Mean Accuracy \%} & \multicolumn{3}{l}{10th Percentile Accuracy \%} \\
{} &          Finetune &            PFL-AM &            PFL-SU &                    Finetune &            PFL-AM &            PFL-SU \\
\midrule
Non-personalized &           $93.18$ &           $93.18$ &           $93.18$ &                     $86.11$ &           $86.11$ &           $86.11$ \\
Input Layer      &           $93.29$ &  $\mathbf{93.38}$ &           $93.36$ &            $\mathbf{86.21}$ &           $86.11$ &  $\mathbf{86.21}$ \\
Output Layer     &           $93.37$ &           $93.37$ &  $\mathbf{93.38}$ &            $\mathbf{86.21}$ &           $86.11$ &  $\mathbf{86.21}$ \\
Adapter          &  $\mathbf{93.65}$ &           $93.63$ &           $93.41$ &                     $86.84$ &  $\mathbf{87.10}$ &           $86.21$ \\
\bottomrule
\end{tabular}


==> tables/per_task/main_pretrained_stateless_gldv2_resnetgn.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{l}{Mean Accuracy \%} & \multicolumn{3}{l}{10th Percentile Accuracy \%} \\
{} &         Finetune &            PFL-AM &   PFL-SU &                    Finetune &            PFL-AM &   PFL-SU \\
\midrule
Non-personalized &          $67.19$ &           $67.19$ &  $67.19$ &                     $53.57$ &           $53.57$ &  $53.57$ \\
Input Layer      &          $67.62$ &  $\mathbf{71.65}$ &  $71.55$ &                     $53.90$ &  $\mathbf{57.69}$ &  $56.91$ \\
Output Layer     &          $69.02$ &  $\mathbf{70.90}$ &  $70.33$ &                     $55.74$ &  $\mathbf{56.25}$ &  $55.74$ \\
Adapter          &          $76.69$ &  $\mathbf{77.68}$ &  $72.66$ &            $\mathbf{63.16}$ &           $61.76$ &  $58.62$ \\
\bottomrule
\end{tabular}


==> tables/per_task/main_pretrained_stateless_so_mini.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{l}{Mean Accuracy \%} & \multicolumn{3}{l}{10th Percentile Accuracy \%} \\
{} &         Finetune &            PFL-AM &   PFL-SU &                    Finetune &            PFL-AM &   PFL-SU \\
\midrule
Non-personalized   &          $23.82$ &           $23.82$ &  $23.82$ &                     $20.17$ &           $20.17$ &  $20.17$ \\
Input Layer        &          $24.95$ &  $\mathbf{25.29}$ &  $24.63$ &                     $21.33$ &  $\mathbf{21.61}$ &  $20.63$ \\
Output Layer       &          $24.92$ &  $\mathbf{25.39}$ &  $24.58$ &                     $21.41$ &  $\mathbf{21.79}$ &  $20.67$ \\
Adapter (dim=$16$) &          $24.71$ &  $\mathbf{25.28}$ &  $24.59$ &                     $21.21$ &  $\mathbf{21.69}$ &  $20.64$ \\
Adapter (dim=$64$) &          $24.73$ &  $\mathbf{25.29}$ &  $24.58$ &                     $21.17$ &  $\mathbf{21.75}$ &  $20.60$ \\
\bottomrule
\end{tabular}


==> tables/per_task/speech_all.tex <==
\begin{tabular}{lrr}
\toprule
{Personalization} &    FedAlt &    FedSim \\
\midrule
Finetune         &  $15.55$ &  $15.55$ \\
Input Layer        &  \tabemph{} $\mathbf{15.13}$ &  $15.47$ \\
Output Layer        &  $15.53$ &  $15.51$ \\
Adapter       &  $15.50$ &  $15.54$ \\
\bottomrule
\end{tabular}



==> tables/per_task/speech_short.tex <==
\begin{tabular}{rrrr}
\toprule
Finetune & Input Layer &  Output Layer &  Adapter \\
\midrule
$15.55$ &   \tabemph{} $\mathbf{15.13}$ &   $15.53$ &    $15.50$ \\
\bottomrule
\end{tabular}



==> tables/pfl-algo_emnist_resnetgn.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{c}{Stateful} & \multicolumn{3}{c}{Stateless} \\
{} &        Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim \\
\midrule
Input Layer  &  $93.29_{0.00}$ &  $\mathbf{93.62}_{0.03}$ &  $93.55_{0.05}$ &  $93.29_{0.00}$ &  $\mathbf{93.51}_{0.03}$ &  $93.48_{0.04}$ \\
Output Layer &  $93.37_{0.01}$ &  $\mathbf{93.57}_{0.04}$ &  $93.55_{0.05}$ &  $93.37_{0.01}$ &  $\mathbf{93.53}_{0.03}$ &  $93.51_{0.04}$ \\
Adapter      &  $93.66_{0.00}$ &  $\mathbf{94.13}_{0.03}$ &  $94.07_{0.03}$ &  $93.66_{0.00}$ &  $\mathbf{93.97}_{0.04}$ &  $93.89_{0.02}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-algo_gldv2b_resnetgn.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{c}{Stateful} & \multicolumn{3}{c}{Stateless} \\
{} &        Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim \\
\midrule
Input Layer  &  $51.97_{0.02}$ &  $\mathbf{53.94}_{0.06}$ &  $53.64_{0.08}$ &  $51.97_{0.02}$ &  $\mathbf{52.76}_{0.06}$ &  $52.74_{0.02}$ \\
Output Layer &  $53.21_{0.01}$ &  $\mathbf{56.64}_{0.05}$ &  $56.24_{0.04}$ &  $53.21_{0.01}$ &  $\mathbf{53.30}_{0.06}$ &  $53.30_{0.08}$ \\
Adapter      &  $63.86_{0.06}$ &  $\mathbf{66.41}_{0.05}$ &  $66.35_{0.03}$ &  $63.86_{0.06}$ &  $\mathbf{64.10}_{0.14}$ &  $63.19_{0.04}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-algo_so_mini.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{c}{Stateful} & \multicolumn{3}{c}{Stateless} \\
{} &                 Finetune &                   FedAlt &          FedSim &                 Finetune &                   FedAlt &          FedSim \\
\midrule
Input Layer        &  $\mathbf{24.96}_{0.01}$ &           $24.44_{0.01}$ &  $24.81_{0.01}$ &  $\mathbf{24.96}_{0.01}$ &           $24.84_{0.01}$ &  $24.89_{0.01}$ \\
Output Layer       &           $24.93_{0.01}$ &  $\mathbf{25.05}_{0.01}$ &  $25.02_{0.01}$ &           $24.93_{0.01}$ &  $\mathbf{24.94}_{0.01}$ &  $24.94_{0.01}$ \\
Adapter (dim=$16$) &           $24.71_{0.00}$ &  $\mathbf{24.82}_{0.01}$ &  $24.74_{0.01}$ &  $\mathbf{24.71}_{0.00}$ &           $24.69_{0.01}$ &  $24.71_{0.01}$ \\
Adapter (dim=$64$) &           $24.74_{0.01}$ &  $\mathbf{24.86}_{0.01}$ &  $24.75_{0.01}$ &  $\mathbf{24.74}_{0.01}$ &           $24.71_{0.01}$ &  $24.73_{0.01}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-full-stateful.tex <==
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} & \multicolumn{3}{c}{EMNIST} \\
{} &                 Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim \\
\midrule
Input Layer  &  $\mathbf{24.96}_{0.01}$ &           $24.44_{0.01}$ &  $24.81_{0.01}$ &  $51.97_{0.02}$ &  $\mathbf{53.94}_{0.06}$ &  $53.64_{0.08}$ &  $93.29_{0.00}$ &  $\mathbf{93.62}_{0.03}$ &  $93.55_{0.05}$ \\
Output Layer &           $24.93_{0.01}$ &  $\mathbf{25.05}_{0.01}$ &  $25.02_{0.01}$ &  $53.21_{0.01}$ &  $\mathbf{56.64}_{0.05}$ &  $56.24_{0.04}$ &  $93.37_{0.01}$ &  $\mathbf{93.57}_{0.04}$ &  $93.55_{0.05}$ \\
Adapter      &           $24.71_{0.00}$ &  $\mathbf{24.82}_{0.01}$ &  $24.74_{0.01}$ &  $63.86_{0.06}$ &  $\mathbf{66.41}_{0.05}$ &  $66.35_{0.03}$ &  $93.66_{0.00}$ &  $\mathbf{94.13}_{0.03}$ &  $94.07_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-full-stateful2-nostd.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} & \multicolumn{3}{c}{EMNIST} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
{} &                 FT (part.) &                   \hlalt{FedAlt} &          \hlsim{FedSim} &        FT (part.) &                   \hlalt{FedAlt} &          \hlsim{FedSim} &        FT (part.) &                   \hlalt{FedAlt} &          \hlsim{FedSim} \\
\midrule
Input Layer  & \tabemph{} $\mathbf{24.96}$ &           $24.44$ &  $24.81$ &  $51.97$ &  \tabemph{}$\mathbf{53.94}$ &  $53.64$ &  $93.29$ &  \tabemph{}$\mathbf{93.62}$ &  $93.55$ \\
Output Layer &           $24.93$ &  \tabemph{}$\mathbf{25.05}$ &  $25.02$ &  $53.21$ &  \tabemph{}$\mathbf{56.64}$ &  $56.24$ &  $93.37$ &  \tabemph{}$\mathbf{93.57}$ &  \tabemph{}$\mathbf{93.55}$ \\
Adapter      &           $24.71$ &  \tabemph{}$\mathbf{24.82}$ &  $24.74$ &  $63.86$ &  \tabemph{}$\mathbf{66.41}$ &  $66.35$ &  $93.66$ &  \tabemph{}$\mathbf{94.13}$ &  $94.07$ \\
\bottomrule
\end{tabular}


==> tables/pfl-full-stateful2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} & \multicolumn{3}{c}{EMNIST} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
{} &                 FT (part.) &                   FedAlt &          FedSim &        FT (part.) &                   FedAlt &          FedSim &        FT (part.) &                   FedAlt &          FedSim \\
\midrule
Input Layer  & \tabemph{} $\mathbf{24.96}_{0.01}$ &           $24.44_{0.01}$ &  $24.81_{0.01}$ &  $51.97_{0.02}$ &  \tabemph{}$\mathbf{53.94}_{0.06}$ &  $53.64_{0.08}$ &  $93.29_{0.00}$ &  \tabemph{}$\mathbf{93.62}_{0.03}$ &  $93.55_{0.05}$ \\
Output Layer &           $24.93_{0.01}$ &  \tabemph{}$\mathbf{25.05}_{0.01}$ &  $25.02_{0.01}$ &  $53.21_{0.01}$ &  \tabemph{}$\mathbf{56.64}_{0.05}$ &  $56.24_{0.04}$ &  $93.37_{0.01}$ &  \tabemph{}$\mathbf{93.57}_{0.04}$ &  \tabemph{}$\mathbf{93.55}_{0.05}$ \\
Adapter      &           $24.71_{0.00}$ &  \tabemph{}$\mathbf{24.82}_{0.01}$ &  $24.74_{0.01}$ &  $63.86_{0.06}$ &  \tabemph{}$\mathbf{66.41}_{0.05}$ &  $66.35_{0.03}$ &  $93.66_{0.00}$ &  \tabemph{}$\mathbf{94.13}_{0.03}$ &  $94.07_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-full-stateless.tex <==
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} & \multicolumn{3}{c}{EMNIST} \\
{} &                 Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim \\
\midrule
Input Layer  &  $\mathbf{24.96}_{0.01}$ &           $24.84_{0.01}$ &  $24.89_{0.01}$ &  $51.97_{0.02}$ &  $\mathbf{52.76}_{0.06}$ &  $52.74_{0.02}$ &  $93.29_{0.00}$ &  $\mathbf{93.51}_{0.03}$ &  $93.48_{0.04}$ \\
Output Layer &           $24.93_{0.01}$ &  $\mathbf{24.94}_{0.01}$ &  $24.94_{0.01}$ &  $53.21_{0.01}$ &  $\mathbf{53.30}_{0.06}$ &  $53.30_{0.08}$ &  $93.37_{0.01}$ &  $\mathbf{93.53}_{0.03}$ &  $93.51_{0.04}$ \\
Adapter      &  $\mathbf{24.71}_{0.00}$ &           $24.69_{0.01}$ &  $24.71_{0.01}$ &  $63.86_{0.06}$ &  $\mathbf{64.10}_{0.14}$ &  $63.19_{0.04}$ &  $93.66_{0.00}$ &  $\mathbf{93.97}_{0.04}$ &  $93.89_{0.02}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-full-stateless2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llllllllll}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} & \multicolumn{3}{c}{EMNIST} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
{} &                 FT (part.) &                   FedAlt &          FedSim &        FT (part.) &                   FedAlt &          FedSim &        FT (part.) &                   FedAlt &          FedSim \\
\midrule
Input Layer  &  \tabemph{}$\mathbf{24.96}_{0.01}$ &           $24.84_{0.01}$ &  $24.89_{0.01}$ &  $51.97_{0.02}$ &  \tabemph{}$\mathbf{52.76}_{0.06}$ &  $52.74_{0.02}$ &  $93.29_{0.00}$ &  \tabemph{}$\mathbf{93.51}_{0.03}$ &  $93.48_{0.04}$ \\
Output Layer &           $24.93_{0.01}$ &  \tabemph{}$\mathbf{24.94}_{0.01}$ &  $24.94_{0.01}$ &  $53.21_{0.01}$ &  \tabemph{}$\mathbf{53.30}_{0.06}$ &  $53.30_{0.08}$ &  $93.37_{0.01}$ &  \tabemph{}$\mathbf{93.53}_{0.03}$ &  $93.51_{0.04}$ \\
Adapter      &  \tabemph{}$\mathbf{24.71}_{0.00}$ &           $24.69_{0.01}$ &  $24.71_{0.01}$ &  $63.86_{0.06}$ &  \tabemph{}$\mathbf{64.10}_{0.14}$ &  $63.19_{0.04}$ &  $93.66_{0.00}$ &  \tabemph{}$\mathbf{93.97}_{0.04}$ &  $93.89_{0.02}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-stateful.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} \\
{} &                 Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim \\
\midrule
Input Layer  &  $\mathbf{24.96}_{0.01}$ &           $24.44_{0.01}$ &  $24.81_{0.01}$ &  $51.97_{0.02}$ &  $\mathbf{53.94}_{0.06}$ &  $53.64_{0.08}$ \\
Output Layer &           $24.93_{0.01}$ &  $\mathbf{25.05}_{0.01}$ &  $25.02_{0.01}$ &  $53.21_{0.01}$ &  $\mathbf{56.64}_{0.05}$ &  $56.24_{0.04}$ \\
Adapter      &           $24.71_{0.00}$ &  $\mathbf{24.82}_{0.01}$ &  $24.74_{0.01}$ &  $63.86_{0.06}$ &  $\mathbf{66.41}_{0.05}$ &  $66.35_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-stateful2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
{} &                 Finetune (part.) &                   \pflam &          \pflsu &        Finetune (part.) &                   \pflam &          \pflsu \\
\midrule
Input Layer  & \tabemph{} $\mathbf{24.96}_{0.01}$ &           $24.44_{0.01}$ &  $24.81_{0.01}$ &  $51.97_{0.02}$ &  \tabemph{}$\mathbf{53.94}_{0.06}$ &  $53.64_{0.08}$ \\
Output Layer &           $24.93_{0.01}$ &  \tabemph{}$\mathbf{25.05}_{0.01}$ &  $25.02_{0.01}$ &  $53.21_{0.01}$ &  \tabemph{}$\mathbf{56.64}_{0.05}$ &  $56.24_{0.04}$ \\
Adapter      &           $24.71_{0.00}$ &  \tabemph{}$\mathbf{24.82}_{0.01}$ &  $24.74_{0.01}$ &  $63.86_{0.06}$ &  \tabemph{}$\mathbf{66.41}_{0.05}$ &  $66.35_{0.03}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-stateless.tex <==
\begin{tabular}{lllllll}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} \\
{} &                 Finetune &                   FedAlt &          FedSim &        Finetune &                   FedAlt &          FedSim \\
\midrule
Input Layer  &  $\mathbf{24.96}_{0.01}$ &           $24.84_{0.01}$ &  $24.89_{0.01}$ &  $51.97_{0.02}$ &  $\mathbf{52.76}_{0.06}$ &  $52.74_{0.02}$ \\
Output Layer &           $24.93_{0.01}$ &  $\mathbf{24.94}_{0.01}$ &  $24.94_{0.01}$ &  $53.21_{0.01}$ &  $\mathbf{53.30}_{0.06}$ &  $53.30_{0.08}$ \\
Adapter      &  $\mathbf{24.71}_{0.00}$ &           $24.69_{0.01}$ &  $24.71_{0.01}$ &  $63.86_{0.06}$ &  $\mathbf{64.10}_{0.14}$ &  $63.19_{0.04}$ \\
\bottomrule
\end{tabular}


==> tables/pfl-stateless2.tex <==
%!TEX root = ../main.tex

\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{3}{c}{StackOverflow} & \multicolumn{3}{c}{GLDv2} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
{} &                 Finetune (part.) &                   \pflam &          \pflsu &        Finetune (part.) &                   \pflam &          \pflsu \\
\midrule
Input Layer  &  \tabemph{} $\mathbf{24.96}_{0.01}$ &           $24.84_{0.01}$ &  $24.89_{0.01}$ &  $51.97_{0.02}$ &  \tabemph{} $\mathbf{52.76}_{0.06}$ &  $52.74_{0.02}$ \\
Output Layer &           $24.93_{0.01}$ &  \tabemph{} $\mathbf{24.94}_{0.01}$ &  \tabemph{} $\mathbf{24.94}_{0.01}$ &  $53.21_{0.01}$ &  \tabemph{} $\mathbf{53.30}_{0.06}$ &  \tabemph{} $\mathbf{53.30}_{0.08}$ \\
Adapter      &  \tabemph{} $\mathbf{24.71}_{0.00}$ &           $24.69_{0.01}$ &  \tabemph{} $\mathbf{24.71}_{0.01}$ &  $63.86_{0.06}$ &  \tabemph{} $\mathbf{64.10}_{0.14}$ &  $63.19_{0.04}$ \\
\bottomrule
\end{tabular}

